Tables as Texts or Images: Evaluating the Table Reasoning Ability of LLMs and MLLMs

In this paper, we investigate the effectiveness of various LLMs in interpreting tabular data through different prompting strategies and data formats. Our analyses extend across six benchmarks for table-related tasks such as question-answering and fact-checking. We introduce for the first time the assessment of LLMs' performance on image-based table representations. Specifically, we compare five text-based and three image-based table representations, demonstrating the role of representation and prompting on LLM performance. Our study provides insights into the effective use of LLMs on table-related tasks.

==> tables/FinQA_test/gemini-pro.tex <==
\begin{tabular}{llll}
\toprule
{} & basic &   CoT & expert \\
\midrule
Linearized\_no\_row\_sign &  0.21 &  0.46 &   0.29 \\
json\_column\_centric    &  0.13 &  0.49 &   0.14 \\
json\_row\_centric       &  0.23 &  0.46 &   0.14 \\
bracket\_format         &  0.21 &  0.56 &   0.23 \\
\bottomrule
\end{tabular}


==> tables/FinQA_test/gpt-35-turbo.tex <==
\begin{tabular}{llll}
\toprule
{} & basic &   CoT & expert \\
\midrule
Linearized\_no\_row\_sign &  0.34 &  0.45 &   0.35 \\
json\_column\_centric    &  0.31 &  0.36 &   0.33 \\
json\_row\_centric       &  0.39 &  0.43 &   0.43 \\
bracket\_format         &  0.37 &  0.43 &    0.3 \\
\bottomrule
\end{tabular}


==> tables/FinQA_test/gpt-4.tex <==
\begin{tabular}{llll}
\toprule
{} & basic &   CoT & expert \\
\midrule
Linearized\_no\_row\_sign &  0.43 &  0.47 &   0.52 \\
json\_column\_centric    &   0.4 &  0.38 &    0.5 \\
json\_row\_centric       &  0.44 &  0.44 &   0.49 \\
bracket\_format         &  0.41 &  0.43 &    0.5 \\
\bottomrule
\end{tabular}


==> tables/FinQA_test/llama-2-13b-chat.tex <==
\begin{tabular}{llll}
\toprule
{} & basic &   CoT & expert \\
\midrule
Linearized\_no\_row\_sign &   0.2 &  0.24 &   0.24 \\
json\_column\_centric    &  0.12 &  0.24 &    0.2 \\
json\_row\_centric       &  0.22 &  0.27 &   0.18 \\
bracket\_format         &  0.26 &  0.29 &   0.26 \\
\bottomrule
\end{tabular}


==> tables/FinQA_test/llama-2-70b-chat.tex <==
\begin{tabular}{llll}
\toprule
{} & basic &   CoT & expert \\
\midrule
Linearized\_no\_row\_sign &  0.41 &  0.47 &    0.4 \\
json\_column\_centric    &  0.37 &  0.43 &   0.35 \\
json\_row\_centric       &  0.36 &  0.44 &   0.42 \\
bracket\_format         &  0.41 &  0.47 &   0.39 \\
\bottomrule
\end{tabular}


==> tables/FinQA_test/llama-2-7b-chat.tex <==
\begin{tabular}{llll}
\toprule
{} & basic &   CoT & expert \\
\midrule
Linearized\_no\_row\_sign &  0.08 &  0.06 &   0.05 \\
json\_column\_centric    &  0.05 &  0.03 &   0.02 \\
json\_row\_centric       &  0.01 &  0.07 &   0.01 \\
bracket\_format         &  0.04 &  0.05 &   0.05 \\
\bottomrule
\end{tabular}


==> tables/Table-Fact-Checking_test/gemini-pro.tex <==
\begin{tabular}{llll}
\toprule
{} &     basic &       CoT &    expert \\
\midrule
Linearized\_no\_row\_sign &  0.645667 &  0.638056 &  0.639778 \\
json\_column\_centric    &  0.639556 &  0.653667 &  0.623167 \\
json\_row\_centric       &  0.640944 &  0.647722 &  0.661278 \\
bracket\_format         &  0.654278 &  0.643389 &  0.634556 \\
\bottomrule
\end{tabular}


==> tables/Table-Fact-Checking_test/gpt-35-turbo.tex <==
\begin{tabular}{llll}
\toprule
{} &     basic &       CoT &    expert \\
\midrule
Linearized\_no\_row\_sign &  0.559833 &  0.560944 &  0.568167 \\
json\_column\_centric    &  0.556722 &  0.559389 &  0.546333 \\
json\_row\_centric       &  0.552278 &  0.540167 &  0.561222 \\
bracket\_format         &  0.573722 &  0.570722 &  0.568833 \\
\bottomrule
\end{tabular}


==> tables/Table-Fact-Checking_test/gpt-4.tex <==
\begin{tabular}{llll}
\toprule
{} &     basic &       CoT &    expert \\
\midrule
Linearized\_no\_row\_sign &  0.715667 &  0.714278 &  0.719722 \\
json\_column\_centric    &  0.714222 &    0.7105 &  0.725722 \\
json\_row\_centric       &  0.738444 &  0.738167 &  0.746667 \\
bracket\_format         &  0.735444 &  0.732222 &  0.737556 \\
\bottomrule
\end{tabular}


==> tables/Table-Fact-Checking_test/llama-2-13b-chat.tex <==
\begin{tabular}{llll}
\toprule
{} &     basic &       CoT &    expert \\
\midrule
Linearized\_no\_row\_sign &     0.464 &  0.422611 &  0.401944 \\
json\_column\_centric    &  0.375667 &  0.350667 &  0.263833 \\
json\_row\_centric       &  0.342333 &  0.367944 &  0.309889 \\
bracket\_format         &  0.432278 &  0.439111 &  0.346833 \\
\bottomrule
\end{tabular}


==> tables/Table-Fact-Checking_test/llama-2-70b-chat.tex <==
\begin{tabular}{llll}
\toprule
{} &     basic &       CoT &    expert \\
\midrule
Linearized\_no\_row\_sign &  0.429778 &  0.462889 &  0.505333 \\
json\_column\_centric    &  0.446333 &  0.471333 &  0.518222 \\
json\_row\_centric       &  0.389222 &  0.388667 &  0.456889 \\
bracket\_format         &  0.418333 &  0.474111 &  0.467833 \\
\bottomrule
\end{tabular}


==> tables/Table-Fact-Checking_test/llama-2-7b-chat.tex <==
\begin{tabular}{llll}
\toprule
{} &     basic &       CoT &    expert \\
\midrule
Linearized\_no\_row\_sign &  0.056556 &  0.063444 &  0.016222 \\
json\_column\_centric    &     0.047 &     0.047 &  0.048444 \\
json\_row\_centric       &     0.057 &  0.052556 &     0.051 \\
bracket\_format         &  0.074556 &     0.069 &     0.018 \\
\bottomrule
\end{tabular}


==> tables/WikiTableQuestions_test/gemini-pro_EM_F1.tex <==
\begin{tabular}{llll}
\toprule
{} &                     basic &                        CoT &                    expert \\
\midrule
Linearized\_no\_row\_sign &  0.46/0.37882738448914915 &   0.65/0.03456768485742019 &  0.33/0.19928195358299722 \\
json\_column\_centric    &  0.34/0.27361507936507934 &   0.61/0.03335155672636856 &   0.3/0.19515695705260921 \\
json\_row\_centric       &  0.52/0.43120893812070277 &  0.71/0.038536504017945464 &    0.44/0.329258062827752 \\
bracket\_format         &  0.48/0.42429551820728295 &   0.69/0.03842878354028043 &   0.39/0.3077792558318874 \\
\bottomrule
\end{tabular}


==> tables/WikiTableQuestions_test/gpt-35-turbo_EM_F1.tex <==
\begin{tabular}{llll}
\toprule
{} &                     basic &                        CoT &                    expert \\
\midrule
Linearized\_no\_row\_sign &  0.63/0.12955823384473333 &   0.68/0.07944925505970969 &  0.62/0.11821759025096633 \\
json\_column\_centric    &   0.6/0.11213268781046812 &  0.72/0.038676334066493984 &  0.62/0.08776495483683584 \\
json\_row\_centric       &  0.58/0.13142164126050226 &   0.72/0.06830068806850285 &  0.63/0.11790410597256441 \\
bracket\_format         &    0.65/0.135973546239274 &   0.67/0.04984757255620956 &   0.6/0.11035639670905555 \\
\bottomrule
\end{tabular}


==> tables/WikiTableQuestions_test/gpt-4_EM_F1.tex <==
\begin{tabular}{llll}
\toprule
{} &                     basic &                       CoT &                    expert \\
\midrule
Linearized\_no\_row\_sign &  0.71/0.16712533330177698 &   0.76/0.1678506749577717 &  0.74/0.14928057184522228 \\
json\_column\_centric    &  0.75/0.17777921740805375 &  0.76/0.15080494254614782 &  0.73/0.14670468497689848 \\
json\_row\_centric       &   0.76/0.1851023002288987 &  0.73/0.16235560640680313 &  0.73/0.15851401177918242 \\
bracket\_format         &    0.71/0.176566273234865 &  0.75/0.15762814158669414 &  0.66/0.14678205471806163 \\
\bottomrule
\end{tabular}


==> tables/WikiTableQuestions_test/llama-2-13b-chat_EM_F1.tex <==
\begin{tabular}{llll}
\toprule
{} &                      basic &                        CoT &                     expert \\
\midrule
Linearized\_no\_row\_sign &    0.4/0.03876915696130969 &   0.43/0.03447993420300353 &  0.31/0.029335277838857678 \\
json\_column\_centric    &  0.26/0.029601151376226258 &  0.33/0.024859093713852278 &   0.31/0.02983933799491499 \\
json\_row\_centric       &    0.31/0.0442493007920521 &   0.4/0.028675919050640947 &    0.4/0.04904285663427841 \\
bracket\_format         &   0.35/0.04072724198376552 &  0.43/0.033887394265440844 &    0.4/0.04067403902783538 \\
\bottomrule
\end{tabular}


==> tables/WikiTableQuestions_test/llama-2-70b-chat_EM_F1.tex <==
\begin{tabular}{llll}
\toprule
{} &                      basic &                        CoT &                     expert \\
\midrule
Linearized\_no\_row\_sign &   0.41/0.05934626255333065 &   0.49/0.05157398058428492 &   0.49/0.06215918963533015 \\
json\_column\_centric    &  0.42/0.054059863389797284 &   0.39/0.03203153399241855 &  0.43/0.045684531284328866 \\
json\_row\_centric       &   0.49/0.07907285133463886 &   0.66/0.05845930462066698 &   0.53/0.07345929731352534 \\
bracket\_format         &    0.44/0.0702829070698032 &  0.59/0.042005146427154215 &    0.49/0.0578750464075053 \\
\bottomrule
\end{tabular}


==> tables/WikiTableQuestions_test/llama-2-7b-chat_EM_F1.tex <==
\begin{tabular}{llll}
\toprule
{} &                      basic &                        CoT &                     expert \\
\midrule
Linearized\_no\_row\_sign &    0.17/0.0210200802013405 &  0.24/0.030419674590431697 &  0.09/0.009892620429995535 \\
json\_column\_centric    &  0.14/0.013557659277352974 &  0.14/0.020816921182175107 &   0.06/0.01232710630810073 \\
json\_row\_centric       &  0.19/0.015368345624733855 &  0.25/0.015267940175222707 &   0.13/0.01291643863974861 \\
bracket\_format         &   0.15/0.01977172638737545 &  0.28/0.030567814903075145 &  0.14/0.023060085387324875 \\
\bottomrule
\end{tabular}


==> tables/all_results_table.tex <==
\begin{table*}[ht]
	\centering
	\begin{adjustbox}{width=\linewidth}
		\begin{tabular}{@{}lccccccc@{}}
			\toprule
			& Metric & Model & Linearized Method &Special Prompt & Results  \\ 
			\midrule
            \multirow{72}*{e2e} 
& bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.03362/0.3492/1.021/0.2859 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Column Centric Json & Basic & 0.09259/0.501/1.775/0.4552 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Row Centric Json & Basic & 0.1071/0.5631/1.85/0.4459 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Bracket Format & Basic & 0.08953/0.5239/1.652/0.4199 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.01663/0.3334/0.6725/0.2127 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Column Centric Json & CoT & 0.08192/0.4904/1.654/0.4374 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Row Centric Json & CoT & 0.09954/0.5492/1.685/0.4361 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Bracket Format & CoT & 0.05133/0.35/0.8641/0.3127 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.0349/0.3413/0.9224/0.2926 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Column Centric Json & Expert & 0.08311/0.4787/1.631/0.4346 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Row Centric Json & Expert & 0.0945/0.5348/1.79/0.4332 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Bracket Format & Expert & 0.08432/0.5053/1.612/0.4171 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/o Row Sign & Basic & 0.08023/0.4641/1.628/0.4483 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Column Centric Json & Basic & 0.08729/0.5059/1.811/0.4562 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Row Centric Json & Basic & 0.09005/0.4959/1.805/0.4571 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Bracket Format & Basic & 0.09035/0.4838/1.744/0.4517 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/o Row Sign & CoT & 0.0819/0.4762/1.704/0.4457 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Column Centric Json & CoT & 0.08406/0.4894/1.691/0.4599 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Row Centric Json & CoT & 0.08366/0.492/1.705/0.4474 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Bracket Format & CoT & 0.07912/0.4899/1.549/0.4242 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/o Row Sign & Expert & 0.08364/0.4652/1.599/0.4492 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Column Centric Json & Expert & 0.08488/0.4907/1.732/0.4512 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Row Centric Json & Expert & 0.08863/0.5028/1.775/0.4495 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Bracket Format & Expert & 0.07867/0.4865/1.645/0.4321 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.04019/0.3933/1.351/0.3564 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Column Centric Json & Basic & 0.06187/0.4585/1.607/0.4159 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Row Centric Json & Basic & 0.02283/0.2669/0.8446/0.2876 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Bracket Format & Basic & 0.01596/0.2752/0.8737/0.2613 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.02777/0.3648/0.5621/0.2109 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Column Centric Json & CoT & 0.02373/0.3499/0.5246/0.2234 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Row Centric Json & CoT & 0.0212/0.3088/0.5003/0.221 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Bracket Format & CoT & 0.01738/0.2874/0.4149/0.1945 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.0552/0.4412/1.406/0.3594 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Column Centric Json & Expert & 0.06945/0.4542/1.595/0.4194 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Row Centric Json & Expert & 0.01697/0.1876/0.6028/0.2188 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Bracket Format & Expert & 0.02709/0.3311/1.086/0.2958 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.008321/0.3034/0.6915/0.2058 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Column Centric Json & Basic & 0.01907/0.2758/0.7319/0.2617 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Row Centric Json & Basic & 0.005682/0.2143/0.6328/0.2149 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Bracket Format & Basic & 0.01089/0.2405/0.703/0.2369 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.005593/0.2931/0.5552/0.177 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Column Centric Json & CoT & 0.01142/0.2389/0.6227/0.2341 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Row Centric Json & CoT & 0.01004/0.2493/0.6738/0.2407 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Bracket Format & CoT & 0.003475/0.2291/0.5886/0.2096 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.01322/0.3201/0.5862/0.2064 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Column Centric Json & Expert & 0.01303/0.2516/0.6443/0.2541 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Row Centric Json & Expert & 0.01364/0.2944/0.7672/0.28 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Bracket Format & Expert & 0.006849/0.252/0.6451/0.2468 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.01218/0.2827/0.6207/0.1997 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Column Centric Json & Basic & 0.0348/0.3697/1.021/0.3141 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Row Centric Json & Basic & 0.01411/0.2542/0.7586/0.259 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Bracket Format & Basic & 0.01737/0.2171/0.6427/0.2124 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.009001/0.2915/0.5192/0.1809 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Column Centric Json & CoT & 0.01122/0.2667/0.5981/0.2321 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Row Centric Json & CoT & 0.003629/0.183/0.3825/0.1927 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Bracket Format & CoT & 0.005145/0.224/0.4808/0.1833 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.006912/0.2588/0.4781/0.1676 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Column Centric Json & Expert & 0.027/0.3331/0.8791/0.2902 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Row Centric Json & Expert & 0.01958/0.2944/0.7631/0.2747 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Bracket Format & Expert & 0.01633/0.264/0.6526/0.2138 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.01356/0.3066/0.715/0.2118 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Column Centric Json & Basic & 0.04892/0.4478/1.354/0.3708 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Row Centric Json & Basic & 0.0307/0.3674/1.009/0.3239 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Bracket Format & Basic & 0.01178/0.2819/0.7667/0.2303 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.01023/0.2718/0.5109/0.167 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Column Centric Json & CoT & 0.0447/0.4022/1.047/0.3005 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Row Centric Json & CoT & 0.02924/0.3218/0.8007/0.2704 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Bracket Format & CoT & 0.0121/0.2309/0.5335/0.1881 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.005513/0.2794/0.4931/0.1584 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Column Centric Json & Expert & 0.02955/0.3742/0.7872/0.2725 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Row Centric Json & Expert & 0.02556/0.3401/0.7928/0.2758 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Bracket Format & Expert & 0.01439/0.2716/0.5939/0.1939 \\
            \midrule
        \multirow{117}*{fetaQA-v1} 
        & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.4451/0.5657/0.3509/0.463/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & Basic & 0.3856/0.498/0.2932/0.4087/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & Basic & 0.4426/0.5674/0.3483/0.4738/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & Basic & 0.4264/0.5632/0.3421/0.4593/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.4437/0.5551/0.3373/0.4588/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.4214/0.421/0.2577/0.35/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & CoT & 0.3158/0.2321/0.1269/0.1963/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & CoT & 0.3998/0.3792/0.2267/0.3196/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & CoT & 0.3862/0.3138/0.1856/0.2655/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.4127/0.3956/0.2386/0.3245/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.4343/0.527/0.312/0.4237/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & Expert & 0.3795/0.4553/0.2615/0.368/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & Expert & 0.4383/0.5418/0.3168/0.4372/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & Expert & 0.43/0.5325/0.3114/0.4225/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.4348/0.5278/0.3053/0.4225/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & Highlighted Cells & 0.484/0.6039/0.3825/0.4912/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & Highlighted Cells & 0.4639/0.598/0.3698/0.4898/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & Highlighted Cells & 0.4902/0.6206/0.396/0.5103/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & Highlighted Cells & 0.4844/0.6104/0.3805/0.4945/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & Highlighted Cells & 0.4875/0.6085/0.3801/0.4905/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & Basic & 0.4613/0.623/0.4059/0.5128/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & Basic & 0.4431/0.6038/0.3918/0.5077/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & Basic & 0.458/0.6203/0.4116/0.5161/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & Basic & 0.4572/0.6235/0.4134/0.5215/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & Basic & 0.4724/0.627/0.4142/0.5231/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & CoT & 0.4781/0.6146/0.4043/0.5057/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & CoT & 0.4409/0.5843/0.3775/0.4868/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & CoT & 0.4654/0.6138/0.4076/0.5139/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & CoT & 0.4674/0.6141/0.4048/0.5132/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & CoT & 0.473/0.6167/0.4061/0.5033/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & Expert & 0.4725/0.6015/0.3859/0.4971/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & Expert & 0.4352/0.5911/0.3709/0.4885/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & Expert & 0.4444/0.5986/0.386/0.493/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & Expert & 0.4551/0.6078/0.3961/0.5073/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & Expert & 0.4661/0.6111/0.3991/0.5047/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & Highlighted Cells & 0.4989/0.6558/0.4368/0.5468/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & Highlighted Cells & 0.4996/0.6643/0.4452/0.5513/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & Highlighted Cells & 0.4902/0.6614/0.4476/0.5542/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & Highlighted Cells & 0.4961/0.6595/0.4478/0.5485/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & Highlighted Cells & 0.5025/0.6625/0.4496/0.5524/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.3717/0.4862/0.2807/0.4017/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & Basic & 0.316/0.4251/0.2334/0.3474/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & Basic & 0.357/0.4889/0.2997/0.4039/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & Basic & 0.3344/0.4822/0.2829/0.3987/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & Basic & 0.337/0.4628/0.2763/0.3924/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.3592/0.3045/0.1552/0.2449/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & CoT & 0.3124/0.2739/0.1382/0.2238/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & CoT & 0.3525/0.2849/0.1584/0.2308/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & CoT & 0.3465/0.2904/0.1577/0.2376/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & CoT & 0.3388/0.2701/0.1366/0.2159/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.3635/0.4528/0.2606/0.376/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & Expert & 0.2602/0.3469/0.1771/0.2874/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & Expert & 0.3479/0.4513/0.253/0.3638/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & Expert & 0.3492/0.4597/0.2543/0.3761/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & Expert & 0.3687/0.4781/0.2819/0.3987/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & Highlighted Cells & 0.4161/0.5413/0.336/0.4405/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & Highlighted Cells & 0.3917/0.5218/0.3133/0.4327/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & Highlighted Cells & 0.3817/0.5276/0.3279/0.4393/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & Highlighted Cells & 0.3987/0.5245/0.3307/0.4494/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & Highlighted Cells & 0.3779/0.5208/0.3212/0.4333/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.387/0.3448/0.1882/0.2764/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & Basic & 0.3471/0.3161/0.1694/0.2591/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & Basic & 0.3781/0.3861/0.2107/0.3065/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & Basic & 0.3724/0.354/0.1972/0.2862/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/ Row Sign & Basic & 0.3803/0.3498/0.1919/0.2817/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.3613/0.3231/0.1723/0.2578/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & CoT & 0.3212/0.2907/0.1523/0.2354/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & CoT & 0.3591/0.3409/0.1811/0.2712/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & CoT & 0.3689/0.3279/0.1839/0.2676/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/ Row Sign & CoT & 0.3671/0.3151/0.1677/0.2484/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.3822/0.3425/0.191/0.2802/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & Expert & 0.339/0.3002/0.1537/0.2377/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & Expert & 0.3667/0.3647/0.1989/0.2943/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & Expert & 0.3787/0.3508/0.1926/0.2795/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & Highlighted Cells & 0.4128/0.3619/0.207/0.2966/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & Highlighted Cells & 0.3733/0.3284/0.1768/0.2714/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & Highlighted Cells & 0.4062/0.3878/0.2228/0.3191/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & Highlighted Cells & 0.4003/0.3745/0.2217/0.3098/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/ Row Sign & Highlighted Cells & 0.3908/0.3385/0.1922/0.2792/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.4086/0.4546/0.2597/0.3645/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & Basic & 0.3906/0.4127/0.2276/0.3275/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & Basic & 0.399/0.4782/0.2687/0.3717/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & Basic & 0.441/0.4645/0.2737/0.3797/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/ Row Sign & Basic & 0.4244/0.4541/0.2622/0.3631/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.3921/0.3668/0.1926/0.2878/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & CoT & 0.3524/0.3051/0.1646/0.2471/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & CoT & 0.368/0.3809/0.2141/0.3047/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & CoT & 0.3982/0.3631/0.2055/0.2963/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/ Row Sign & CoT & 0.3953/0.3967/0.2245/0.3142/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.4164/0.4309/0.244/0.3427/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & Expert & 0.3676/0.3726/0.2084/0.2974/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & Expert & 0.4022/0.419/0.2415/0.3449/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & Expert & 0.424/0.4318/0.2559/0.349/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & Highlighted Cells & 0.4474/0.4644/0.2773/0.3735/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & Highlighted Cells & 0.4247/0.4344/0.2528/0.3517/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & Highlighted Cells & 0.439/0.4811/0.2797/0.3887/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & Highlighted Cells & 0.4387/0.4533/0.2702/0.3617/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/ Row Sign & Highlighted Cells & 0.4145/0.4481/0.2537/0.364/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.3762/0.3727/0.2092/0.3015/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & Basic & 0.3466/0.3545/0.189/0.2923/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & Basic & 0.3798/0.4/0.2234/0.3223/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & Basic & 0.3751/0.371/0.2094/0.3001/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/ Row Sign & Basic & 0.3678/0.369/0.2137/0.3042/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.3594/0.3127/0.1813/0.2588/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & CoT & 0.3291/0.2942/0.1582/0.2432/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & CoT & 0.3523/0.333/0.1895/0.2721/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & CoT & 0.3613/0.3199/0.179/0.261/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/ Row Sign & CoT & 0.3672/0.3271/0.1894/0.2651/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.3717/0.3485/0.2013/0.2822/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & Expert & 0.3267/0.3098/0.1635/0.2569/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & Expert & 0.3643/0.3655/0.2056/0.2997/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & Expert & 0.3678/0.3496/0.1974/0.2827/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & Highlighted Cells & 0.4028/0.3824/0.2231/0.3089/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & Highlighted Cells & 0.3812/0.3656/0.2081/0.3019/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & Highlighted Cells & 0.3991/0.4138/0.2434/0.3406/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & Highlighted Cells & 0.3784/0.3693/0.2106/0.3006/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/ Row Sign & Highlighted Cells & 0.3903/0.3623/0.2076/0.2983/0 \\
            \midrule
        \multirow{117}*{FinQA} 
        & Acc & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.34 \\
            & Acc & GPT-3.5-Turbo & Column Centric Json & Basic & 0.31 \\
            & Acc & GPT-3.5-Turbo & Row Centric Json & Basic & 0.39 \\
            & Acc & GPT-3.5-Turbo & Bracket Format & Basic & 0.37 \\
            & Acc & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.37 \\
            & Acc & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.45 \\
            & Acc & GPT-3.5-Turbo & Column Centric Json & CoT & 0.36 \\
            & Acc & GPT-3.5-Turbo & Row Centric Json & CoT & 0.43 \\
            & Acc & GPT-3.5-Turbo & Bracket Format & CoT & 0.43 \\
            & Acc & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.42 \\
            & Acc & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.35 \\
            & Acc & GPT-3.5-Turbo & Column Centric Json & Expert & 0.33 \\
            & Acc & GPT-3.5-Turbo & Row Centric Json & Expert & 0.43 \\
            & Acc & GPT-3.5-Turbo & Bracket Format & Expert & 0.3 \\
            & Acc & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.38 \\
            & Acc & GPT-3.5-Turbo & Linearized w/o Row Sign & Highlighted Cells & 0.3 \\
            & Acc & GPT-3.5-Turbo & Column Centric Json & Highlighted Cells & 0.38 \\
            & Acc & GPT-3.5-Turbo & Row Centric Json & Highlighted Cells & 0.34 \\
            & Acc & GPT-3.5-Turbo & Bracket Format & Highlighted Cells & 0.35 \\
            & Acc & GPT-3.5-Turbo & Linearized w/ Row Sign & Highlighted Cells & 0.33 \\
            & Acc & GPT-4 & Linearized w/o Row Sign & Basic & 0.43 \\
            & Acc & GPT-4 & Column Centric Json & Basic & 0.4 \\
            & Acc & GPT-4 & Row Centric Json & Basic & 0.44 \\
            & Acc & GPT-4 & Bracket Format & Basic & 0.41 \\
            & Acc & GPT-4 & Linearized w/ Row Sign & Basic & 0.44 \\
            & Acc & GPT-4 & Linearized w/o Row Sign & CoT & 0.47 \\
            & Acc & GPT-4 & Column Centric Json & CoT & 0.38 \\
            & Acc & GPT-4 & Row Centric Json & CoT & 0.44 \\
            & Acc & GPT-4 & Bracket Format & CoT & 0.43 \\
            & Acc & GPT-4 & Linearized w/ Row Sign & CoT & 0.44 \\
            & Acc & GPT-4 & Linearized w/o Row Sign & Expert & 0.52 \\
            & Acc & GPT-4 & Column Centric Json & Expert & 0.5 \\
            & Acc & GPT-4 & Row Centric Json & Expert & 0.49 \\
            & Acc & GPT-4 & Bracket Format & Expert & 0.5 \\
            & Acc & GPT-4 & Linearized w/ Row Sign & Expert & 0.5 \\
            & Acc & GPT-4 & Linearized w/o Row Sign & Highlighted Cells & 0.51 \\
            & Acc & GPT-4 & Column Centric Json & Highlighted Cells & 0.46 \\
            & Acc & GPT-4 & Row Centric Json & Highlighted Cells & 0.47 \\
            & Acc & GPT-4 & Bracket Format & Highlighted Cells & 0.49 \\
            & Acc & GPT-4 & Linearized w/ Row Sign & Highlighted Cells & 0.48 \\
            & Acc & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.21 \\
            & Acc & Gemini-Pro & Column Centric Json & Basic & 0.13 \\
            & Acc & Gemini-Pro & Row Centric Json & Basic & 0.23 \\
            & Acc & Gemini-Pro & Bracket Format & Basic & 0.21 \\
            & Acc & Gemini-Pro & Linearized w/ Row Sign & Basic & 0.28 \\
            & Acc & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.46 \\
            & Acc & Gemini-Pro & Column Centric Json & CoT & 0.49 \\
            & Acc & Gemini-Pro & Row Centric Json & CoT & 0.46 \\
            & Acc & Gemini-Pro & Bracket Format & CoT & 0.56 \\
            & Acc & Gemini-Pro & Linearized w/ Row Sign & CoT & 0.53 \\
            & Acc & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.29 \\
            & Acc & Gemini-Pro & Column Centric Json & Expert & 0.14 \\
            & Acc & Gemini-Pro & Row Centric Json & Expert & 0.14 \\
            & Acc & Gemini-Pro & Bracket Format & Expert & 0.23 \\
            & Acc & Gemini-Pro & Linearized w/ Row Sign & Expert & 0.23 \\
            & Acc & Gemini-Pro & Linearized w/o Row Sign & Highlighted Cells & 0.25 \\
            & Acc & Gemini-Pro & Column Centric Json & Highlighted Cells & 0.25 \\
            & Acc & Gemini-Pro & Row Centric Json & Highlighted Cells & 0.35 \\
            & Acc & Gemini-Pro & Bracket Format & Highlighted Cells & 0.26 \\
            & Acc & Gemini-Pro & Linearized w/ Row Sign & Highlighted Cells & 0.26 \\
            & Acc & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.2 \\
            & Acc & LLAMA-2-13B & Column Centric Json & Basic & 0.12 \\
            & Acc & LLAMA-2-13B & Row Centric Json & Basic & 0.22 \\
            & Acc & LLAMA-2-13B & Bracket Format & Basic & 0.26 \\
            & Acc & LLAMA-2-13B & Linearized w/ Row Sign & Basic & 0.24 \\
            & Acc & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.24 \\
            & Acc & LLAMA-2-13B & Column Centric Json & CoT & 0.24 \\
            & Acc & LLAMA-2-13B & Row Centric Json & CoT & 0.27 \\
            & Acc & LLAMA-2-13B & Bracket Format & CoT & 0.29 \\
            & Acc & LLAMA-2-13B & Linearized w/ Row Sign & CoT & 0.18 \\
            & Acc & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.24 \\
            & Acc & LLAMA-2-13B & Column Centric Json & Expert & 0.2 \\
            & Acc & LLAMA-2-13B & Row Centric Json & Expert & 0.18 \\
            & Acc & LLAMA-2-13B & Bracket Format & Expert & 0.26 \\
            & Acc & LLAMA-2-13B & Linearized w/o Row Sign & Highlighted Cells & 0.16 \\
            & Acc & LLAMA-2-13B & Column Centric Json & Highlighted Cells & 0.23 \\
            & Acc & LLAMA-2-13B & Row Centric Json & Highlighted Cells & 0.19 \\
            & Acc & LLAMA-2-13B & Bracket Format & Highlighted Cells & 0.23 \\
            & Acc & LLAMA-2-13B & Linearized w/ Row Sign & Highlighted Cells & 0.2 \\
            & Acc & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.41 \\
            & Acc & LLAMA-2-70B & Column Centric Json & Basic & 0.37 \\
            & Acc & LLAMA-2-70B & Row Centric Json & Basic & 0.36 \\
            & Acc & LLAMA-2-70B & Bracket Format & Basic & 0.41 \\
            & Acc & LLAMA-2-70B & Linearized w/ Row Sign & Basic & 0.39 \\
            & Acc & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.47 \\
            & Acc & LLAMA-2-70B & Column Centric Json & CoT & 0.43 \\
            & Acc & LLAMA-2-70B & Row Centric Json & CoT & 0.44 \\
            & Acc & LLAMA-2-70B & Bracket Format & CoT & 0.47 \\
            & Acc & LLAMA-2-70B & Linearized w/ Row Sign & CoT & 0.35 \\
            & Acc & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.4 \\
            & Acc & LLAMA-2-70B & Column Centric Json & Expert & 0.35 \\
            & Acc & LLAMA-2-70B & Row Centric Json & Expert & 0.42 \\
            & Acc & LLAMA-2-70B & Bracket Format & Expert & 0.39 \\
            & Acc & LLAMA-2-70B & Linearized w/o Row Sign & Highlighted Cells & 0.37 \\
            & Acc & LLAMA-2-70B & Column Centric Json & Highlighted Cells & 0.39 \\
            & Acc & LLAMA-2-70B & Row Centric Json & Highlighted Cells & 0.36 \\
            & Acc & LLAMA-2-70B & Bracket Format & Highlighted Cells & 0.41 \\
            & Acc & LLAMA-2-70B & Linearized w/ Row Sign & Highlighted Cells & 0.37 \\
            & Acc & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.1 \\
            & Acc & LLAMA-2-7B & Column Centric Json & Basic & 0.11 \\
            & Acc & LLAMA-2-7B & Row Centric Json & Basic & 0.18 \\
            & Acc & LLAMA-2-7B & Bracket Format & Basic & 0.12 \\
            & Acc & LLAMA-2-7B & Linearized w/ Row Sign & Basic & 0.09 \\
            & Acc & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.15 \\
            & Acc & LLAMA-2-7B & Column Centric Json & CoT & 0.1 \\
            & Acc & LLAMA-2-7B & Row Centric Json & CoT & 0.14 \\
            & Acc & LLAMA-2-7B & Bracket Format & CoT & 0.22 \\
            & Acc & LLAMA-2-7B & Linearized w/ Row Sign & CoT & 0.14 \\
            & Acc & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.11 \\
            & Acc & LLAMA-2-7B & Column Centric Json & Expert & 0.11 \\
            & Acc & LLAMA-2-7B & Row Centric Json & Expert & 0.09 \\
            & Acc & LLAMA-2-7B & Bracket Format & Expert & 0.1 \\
            & Acc & LLAMA-2-7B & Linearized w/o Row Sign & Highlighted Cells & 0.14 \\
            & Acc & LLAMA-2-7B & Column Centric Json & Highlighted Cells & 0.17 \\
            & Acc & LLAMA-2-7B & Row Centric Json & Highlighted Cells & 0.13 \\
            & Acc & LLAMA-2-7B & Bracket Format & Highlighted Cells & 0.17 \\
            & Acc & LLAMA-2-7B & Linearized w/ Row Sign & Highlighted Cells & 0.11 \\
            \midrule
\multirow{30}*{HybridQA} 
& EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.16/0.04124 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & Basic & 0.13/0.0298 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & Basic & 0.11/0.0306 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & Basic & 0.09/0.02818 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.17/0.04162 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.19/0.0354 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & CoT & 0.19/0.01296 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & CoT & 0.16/0.02264 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & CoT & 0.15/0.01517 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.18/0.03306 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.14/0.03961 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & Expert & 0.18/0.0366 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & Expert & 0.09/0.02099 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & Expert & 0.09/0.02428 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.15/0.04228 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & Basic & 0.14/0.03912 \\
            & EM/F1 & GPT-4 & Column Centric Json & Basic & 0.18/0.04793 \\
            & EM/F1 & GPT-4 & Row Centric Json & Basic & 0.11/0.03135 \\
            & EM/F1 & GPT-4 & Bracket Format & Basic & 0.12/0.03631 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & Basic & 0.12/0.03699 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & CoT & 0.14/0.04119 \\
            & EM/F1 & GPT-4 & Column Centric Json & CoT & 0.15/0.04033 \\
            & EM/F1 & GPT-4 & Row Centric Json & CoT & 0.1/0.03157 \\
            & EM/F1 & GPT-4 & Bracket Format & CoT & 0.13/0.03325 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & CoT & 0.12/0.03495 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & Expert & 0.16/0.03795 \\
            & EM/F1 & GPT-4 & Column Centric Json & Expert & 0.15/0.03566 \\
            & EM/F1 & GPT-4 & Row Centric Json & Expert & 0.09/0.02745 \\
            & EM/F1 & GPT-4 & Bracket Format & Expert & 0.1/0.02936 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & Expert & 0.12/0.03232 \\
            \midrule
\multirow{117}*{LogicNLG} 
& meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.4451/0.5657/0.3509/0.463/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & Basic & 0.3856/0.498/0.2932/0.4087/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & Basic & 0.4426/0.5674/0.3483/0.4738/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & Basic & 0.4264/0.5632/0.3421/0.4593/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.4437/0.5551/0.3373/0.4588/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.4214/0.421/0.2577/0.35/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & CoT & 0.3158/0.2321/0.1269/0.1963/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & CoT & 0.3998/0.3792/0.2267/0.3196/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & CoT & 0.3862/0.3138/0.1856/0.2655/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.4127/0.3956/0.2386/0.3245/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.4343/0.527/0.312/0.4237/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & Expert & 0.3795/0.4553/0.2615/0.368/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & Expert & 0.4383/0.5418/0.3168/0.4372/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & Expert & 0.43/0.5325/0.3114/0.4225/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.4348/0.5278/0.3053/0.4225/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/o Row Sign & Highlighted Cells & 0.484/0.6039/0.3825/0.4912/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Column Centric Json & Highlighted Cells & 0.4639/0.598/0.3698/0.4898/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Row Centric Json & Highlighted Cells & 0.4902/0.6206/0.396/0.5103/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Bracket Format & Highlighted Cells & 0.4844/0.6104/0.3805/0.4945/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-3.5-Turbo & Linearized w/ Row Sign & Highlighted Cells & 0.4875/0.6085/0.3801/0.4905/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & Basic & 0.4613/0.623/0.4059/0.5128/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & Basic & 0.4431/0.6038/0.3918/0.5077/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & Basic & 0.458/0.6203/0.4116/0.5161/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & Basic & 0.4572/0.6235/0.4134/0.5215/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & Basic & 0.4724/0.627/0.4142/0.5231/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & CoT & 0.4781/0.6146/0.4043/0.5057/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & CoT & 0.4409/0.5843/0.3775/0.4868/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & CoT & 0.4654/0.6138/0.4076/0.5139/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & CoT & 0.4674/0.6141/0.4048/0.5132/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & CoT & 0.473/0.6167/0.4061/0.5033/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & Expert & 0.4725/0.6015/0.3859/0.4971/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & Expert & 0.4352/0.5911/0.3709/0.4885/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & Expert & 0.4444/0.5986/0.386/0.493/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & Expert & 0.4551/0.6078/0.3961/0.5073/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & Expert & 0.4661/0.6111/0.3991/0.5047/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/o Row Sign & Highlighted Cells & 0.4989/0.6558/0.4368/0.5468/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Column Centric Json & Highlighted Cells & 0.4996/0.6643/0.4452/0.5513/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Row Centric Json & Highlighted Cells & 0.4902/0.6614/0.4476/0.5542/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Bracket Format & Highlighted Cells & 0.4961/0.6595/0.4478/0.5485/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & GPT-4 & Linearized w/ Row Sign & Highlighted Cells & 0.5025/0.6625/0.4496/0.5524/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.3717/0.4862/0.2807/0.4017/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & Basic & 0.316/0.4251/0.2334/0.3474/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & Basic & 0.357/0.4889/0.2997/0.4039/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & Basic & 0.3344/0.4822/0.2829/0.3987/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & Basic & 0.337/0.4628/0.2763/0.3924/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.3592/0.3045/0.1552/0.2449/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & CoT & 0.3124/0.2739/0.1382/0.2238/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & CoT & 0.3525/0.2849/0.1584/0.2308/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & CoT & 0.3465/0.2904/0.1577/0.2376/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & CoT & 0.3388/0.2701/0.1366/0.2159/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.3635/0.4528/0.2606/0.376/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & Expert & 0.2602/0.3469/0.1771/0.2874/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & Expert & 0.3479/0.4513/0.253/0.3638/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & Expert & 0.3492/0.4597/0.2543/0.3761/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & Expert & 0.3687/0.4781/0.2819/0.3987/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/o Row Sign & Highlighted Cells & 0.4161/0.5413/0.336/0.4405/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Column Centric Json & Highlighted Cells & 0.3917/0.5218/0.3133/0.4327/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Row Centric Json & Highlighted Cells & 0.3817/0.5276/0.3279/0.4393/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Bracket Format & Highlighted Cells & 0.3987/0.5245/0.3307/0.4494/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & Gemini-Pro & Linearized w/ Row Sign & Highlighted Cells & 0.3779/0.5208/0.3212/0.4333/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.387/0.3448/0.1882/0.2764/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & Basic & 0.3471/0.3161/0.1694/0.2591/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & Basic & 0.3781/0.3861/0.2107/0.3065/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & Basic & 0.3724/0.354/0.1972/0.2862/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/ Row Sign & Basic & 0.3803/0.3498/0.1919/0.2817/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.3613/0.3231/0.1723/0.2578/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & CoT & 0.3212/0.2907/0.1523/0.2354/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & CoT & 0.3591/0.3409/0.1811/0.2712/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & CoT & 0.3689/0.3279/0.1839/0.2676/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/ Row Sign & CoT & 0.3671/0.3151/0.1677/0.2484/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.3822/0.3425/0.191/0.2802/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & Expert & 0.339/0.3002/0.1537/0.2377/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & Expert & 0.3667/0.3647/0.1989/0.2943/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & Expert & 0.3787/0.3508/0.1926/0.2795/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/o Row Sign & Highlighted Cells & 0.4128/0.3619/0.207/0.2966/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Column Centric Json & Highlighted Cells & 0.3733/0.3284/0.1768/0.2714/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Row Centric Json & Highlighted Cells & 0.4062/0.3878/0.2228/0.3191/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Bracket Format & Highlighted Cells & 0.4003/0.3745/0.2217/0.3098/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-13B & Linearized w/ Row Sign & Highlighted Cells & 0.3908/0.3385/0.1922/0.2792/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.4086/0.4546/0.2597/0.3645/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & Basic & 0.3906/0.4127/0.2276/0.3275/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & Basic & 0.399/0.4782/0.2687/0.3717/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & Basic & 0.441/0.4645/0.2737/0.3797/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/ Row Sign & Basic & 0.4244/0.4541/0.2622/0.3631/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.3921/0.3668/0.1926/0.2878/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & CoT & 0.3524/0.3051/0.1646/0.2471/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & CoT & 0.368/0.3809/0.2141/0.3047/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & CoT & 0.3982/0.3631/0.2055/0.2963/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/ Row Sign & CoT & 0.3953/0.3967/0.2245/0.3142/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.4164/0.4309/0.244/0.3427/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & Expert & 0.3676/0.3726/0.2084/0.2974/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & Expert & 0.4022/0.419/0.2415/0.3449/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & Expert & 0.424/0.4318/0.2559/0.349/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/o Row Sign & Highlighted Cells & 0.4474/0.4644/0.2773/0.3735/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Column Centric Json & Highlighted Cells & 0.4247/0.4344/0.2528/0.3517/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Row Centric Json & Highlighted Cells & 0.439/0.4811/0.2797/0.3887/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Bracket Format & Highlighted Cells & 0.4387/0.4533/0.2702/0.3617/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-70B & Linearized w/ Row Sign & Highlighted Cells & 0.4145/0.4481/0.2537/0.364/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.3762/0.3727/0.2092/0.3015/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & Basic & 0.3466/0.3545/0.189/0.2923/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & Basic & 0.3798/0.4/0.2234/0.3223/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & Basic & 0.3751/0.371/0.2094/0.3001/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/ Row Sign & Basic & 0.3678/0.369/0.2137/0.3042/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.3594/0.3127/0.1813/0.2588/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & CoT & 0.3291/0.2942/0.1582/0.2432/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & CoT & 0.3523/0.333/0.1895/0.2721/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & CoT & 0.3613/0.3199/0.179/0.261/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/ Row Sign & CoT & 0.3672/0.3271/0.1894/0.2651/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.3717/0.3485/0.2013/0.2822/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & Expert & 0.3267/0.3098/0.1635/0.2569/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & Expert & 0.3643/0.3655/0.2056/0.2997/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & Expert & 0.3678/0.3496/0.1974/0.2827/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/o Row Sign & Highlighted Cells & 0.4028/0.3824/0.2231/0.3089/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Column Centric Json & Highlighted Cells & 0.3812/0.3656/0.2081/0.3019/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Row Centric Json & Highlighted Cells & 0.3991/0.4138/0.2434/0.3406/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Bracket Format & Highlighted Cells & 0.3784/0.3693/0.2106/0.3006/0 \\
            & meteor/rouge1/rouge2/rougeL/scarebleu & LLAMA-2-7B & Linearized w/ Row Sign & Highlighted Cells & 0.3903/0.3623/0.2076/0.2983/0 \\
            \midrule
\multirow{87}*{Table-Fact-Checking} 
& Acc & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.5598333333333335 \\
            & Acc & GPT-3.5-Turbo & Column Centric Json & Basic & 0.5567222222222225 \\
            & Acc & GPT-3.5-Turbo & Row Centric Json & Basic & 0.5522777777777779 \\
            & Acc & GPT-3.5-Turbo & Bracket Format & Basic & 0.5737222222222226 \\
            & Acc & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.5598333333333335 \\
            & Acc & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.5609444444444447 \\
            & Acc & GPT-3.5-Turbo & Column Centric Json & CoT & 0.5593888888888892 \\
            & Acc & GPT-3.5-Turbo & Row Centric Json & CoT & 0.5401666666666669 \\
            & Acc & GPT-3.5-Turbo & Bracket Format & CoT & 0.5707222222222226 \\
            & Acc & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.5663333333333337 \\
            & Acc & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.568166666666667 \\
            & Acc & GPT-3.5-Turbo & Column Centric Json & Expert & 0.5463333333333334 \\
            & Acc & GPT-3.5-Turbo & Row Centric Json & Expert & 0.5612222222222225 \\
            & Acc & GPT-3.5-Turbo & Bracket Format & Expert & 0.5688333333333336 \\
            & Acc & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.5690555555555561 \\
            & Acc & GPT-4 & Linearized w/o Row Sign & Basic & 0.7156666666666665 \\
            & Acc & GPT-4 & Column Centric Json & Basic & 0.7142222222222219 \\
            & Acc & GPT-4 & Row Centric Json & Basic & 0.7384444444444443 \\
            & Acc & GPT-4 & Bracket Format & Basic & 0.7354444444444441 \\
            & Acc & GPT-4 & Linearized w/ Row Sign & Basic & 0.7333333333333333 \\
            & Acc & GPT-4 & Linearized w/o Row Sign & CoT & 0.7142777777777778 \\
            & Acc & GPT-4 & Column Centric Json & CoT & 0.7105 \\
            & Acc & GPT-4 & Row Centric Json & CoT & 0.7381666666666663 \\
            & Acc & GPT-4 & Bracket Format & CoT & 0.732222222222222 \\
            & Acc & GPT-4 & Linearized w/ Row Sign & CoT & 0.7196111111111106 \\
            & Acc & GPT-4 & Linearized w/o Row Sign & Expert & 0.7197222222222222 \\
            & Acc & GPT-4 & Column Centric Json & Expert & 0.7257222222222223 \\
            & Acc & GPT-4 & Row Centric Json & Expert & 0.7466666666666666 \\
            & Acc & GPT-4 & Bracket Format & Expert & 0.7375555555555553 \\
            & Acc & GPT-4 & Linearized w/ Row Sign & Expert & 0.7307222222222223 \\
            & Acc & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.6456666666666669 \\
            & Acc & Gemini-Pro & Column Centric Json & Basic & 0.6395555555555557 \\
            & Acc & Gemini-Pro & Row Centric Json & Basic & 0.6409444444444446 \\
            & Acc & Gemini-Pro & Bracket Format & Basic & 0.6542777777777775 \\
            & Acc & Gemini-Pro & Linearized w/ Row Sign & Basic & 0.6605 \\
            & Acc & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.6380555555555558 \\
            & Acc & Gemini-Pro & Column Centric Json & CoT & 0.6536666666666672 \\
            & Acc & Gemini-Pro & Row Centric Json & CoT & 0.6477222222222221 \\
            & Acc & Gemini-Pro & Bracket Format & CoT & 0.643388888888889 \\
            & Acc & Gemini-Pro & Linearized w/ Row Sign & CoT & 0.6482777777777781 \\
            & Acc & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.639777777777778 \\
            & Acc & Gemini-Pro & Column Centric Json & Expert & 0.6231666666666666 \\
            & Acc & Gemini-Pro & Row Centric Json & Expert & 0.6612777777777781 \\
            & Acc & Gemini-Pro & Bracket Format & Expert & 0.6345555555555557 \\
            & Acc & Gemini-Pro & Linearized w/ Row Sign & Expert & 0.6451111111111111 \\
            & Acc & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.46399999999999997 \\
            & Acc & LLAMA-2-13B & Column Centric Json & Basic & 0.37566666666666676 \\
            & Acc & LLAMA-2-13B & Row Centric Json & Basic & 0.34233333333333343 \\
            & Acc & LLAMA-2-13B & Bracket Format & Basic & 0.4322777777777778 \\
            & Acc & LLAMA-2-13B & Linearized w/ Row Sign & Basic & 0.40494444444444455 \\
            & Acc & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.4226111111111111 \\
            & Acc & LLAMA-2-13B & Column Centric Json & CoT & 0.3506666666666667 \\
            & Acc & LLAMA-2-13B & Row Centric Json & CoT & 0.36794444444444446 \\
            & Acc & LLAMA-2-13B & Bracket Format & CoT & 0.43911111111111106 \\
            & Acc & LLAMA-2-13B & Linearized w/ Row Sign & CoT & 0.3441111111111112 \\
            & Acc & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.40194444444444444 \\
            & Acc & LLAMA-2-13B & Column Centric Json & Expert & 0.26383333333333336 \\
            & Acc & LLAMA-2-13B & Row Centric Json & Expert & 0.3098888888888888 \\
            & Acc & LLAMA-2-13B & Bracket Format & Expert & 0.3468333333333335 \\
            & Acc & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.42977777777777776 \\
            & Acc & LLAMA-2-70B & Column Centric Json & Basic & 0.4463333333333334 \\
            & Acc & LLAMA-2-70B & Row Centric Json & Basic & 0.3892222222222223 \\
            & Acc & LLAMA-2-70B & Bracket Format & Basic & 0.41833333333333356 \\
            & Acc & LLAMA-2-70B & Linearized w/ Row Sign & Basic & 0.4612222222222225 \\
            & Acc & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.4628888888888891 \\
            & Acc & LLAMA-2-70B & Column Centric Json & CoT & 0.4713333333333336 \\
            & Acc & LLAMA-2-70B & Row Centric Json & CoT & 0.3886666666666667 \\
            & Acc & LLAMA-2-70B & Bracket Format & CoT & 0.4741111111111111 \\
            & Acc & LLAMA-2-70B & Linearized w/ Row Sign & CoT & 0.4708888888888892 \\
            & Acc & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.5053333333333334 \\
            & Acc & LLAMA-2-70B & Column Centric Json & Expert & 0.5182222222222223 \\
            & Acc & LLAMA-2-70B & Row Centric Json & Expert & 0.45688888888888923 \\
            & Acc & LLAMA-2-70B & Bracket Format & Expert & 0.46783333333333343 \\
            & Acc & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.5042222222222223 \\
            & Acc & LLAMA-2-7B & Column Centric Json & Basic & 0.4483333333333334 \\
            & Acc & LLAMA-2-7B & Row Centric Json & Basic & 0.43083333333333335 \\
            & Acc & LLAMA-2-7B & Bracket Format & Basic & 0.4863333333333334 \\
            & Acc & LLAMA-2-7B & Linearized w/ Row Sign & Basic & 0.4530555555555557 \\
            & Acc & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.4632222222222224 \\
            & Acc & LLAMA-2-7B & Column Centric Json & CoT & 0.4526111111111113 \\
            & Acc & LLAMA-2-7B & Row Centric Json & CoT & 0.3894444444444444 \\
            & Acc & LLAMA-2-7B & Bracket Format & CoT & 0.4722222222222224 \\
            & Acc & LLAMA-2-7B & Linearized w/ Row Sign & CoT & 0.43833333333333335 \\
            & Acc & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.3864444444444446 \\
            & Acc & LLAMA-2-7B & Column Centric Json & Expert & 0.4098888888888891 \\
            & Acc & LLAMA-2-7B & Row Centric Json & Expert & 0.39455555555555555 \\
            & Acc & LLAMA-2-7B & Bracket Format & Expert & 0.4285000000000001 \\
            \midrule
\multirow{87}*{tatqa} 
& EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.31/0.1194 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & Basic & 0.28/0.1082 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & Basic & 0.31/0.1148 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & Basic & 0.35/0.1229 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.31/0.1174 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.33/0.0764 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & CoT & 0.29/0.07685 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & CoT & 0.35/0.08358 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & CoT & 0.32/0.07679 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.34/0.07597 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.31/0.1047 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & Expert & 0.29/0.1126 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & Expert & 0.31/0.1081 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & Expert & 0.36/0.11 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.35/0.1013 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & Basic & 0.34/0.17 \\
            & EM/F1 & GPT-4 & Column Centric Json & Basic & 0.31/0.1607 \\
            & EM/F1 & GPT-4 & Row Centric Json & Basic & 0.31/0.1678 \\
            & EM/F1 & GPT-4 & Bracket Format & Basic & 0.35/0.1804 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & Basic & 0.34/0.1739 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & CoT & 0.32/0.1656 \\
            & EM/F1 & GPT-4 & Column Centric Json & CoT & 0.3/0.154 \\
            & EM/F1 & GPT-4 & Row Centric Json & CoT & 0.3/0.1607 \\
            & EM/F1 & GPT-4 & Bracket Format & CoT & 0.36/0.1788 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & CoT & 0.31/0.1665 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & Expert & 0.36/0.1673 \\
            & EM/F1 & GPT-4 & Column Centric Json & Expert & 0.31/0.151 \\
            & EM/F1 & GPT-4 & Row Centric Json & Expert & 0.33/0.1556 \\
            & EM/F1 & GPT-4 & Bracket Format & Expert & 0.36/0.1736 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & Expert & 0.35/0.1649 \\
            & EM/F1 & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.27/0.3071 \\
            & EM/F1 & Gemini-Pro & Column Centric Json & Basic & 0.3/0.3108 \\
            & EM/F1 & Gemini-Pro & Row Centric Json & Basic & 0.31/0.3045 \\
            & EM/F1 & Gemini-Pro & Bracket Format & Basic & 0.36/0.3647 \\
            & EM/F1 & Gemini-Pro & Linearized w/ Row Sign & Basic & 0.32/0.3064 \\
            & EM/F1 & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.33/0.09913 \\
            & EM/F1 & Gemini-Pro & Column Centric Json & CoT & 0.34/0.1125 \\
            & EM/F1 & Gemini-Pro & Row Centric Json & CoT & 0.33/0.08826 \\
            & EM/F1 & Gemini-Pro & Bracket Format & CoT & 0.43/0.1446 \\
            & EM/F1 & Gemini-Pro & Linearized w/ Row Sign & CoT & 0.28/0.07928 \\
            & EM/F1 & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.3/0.2866 \\
            & EM/F1 & Gemini-Pro & Column Centric Json & Expert & 0.24/0.2693 \\
            & EM/F1 & Gemini-Pro & Row Centric Json & Expert & 0.29/0.2704 \\
            & EM/F1 & Gemini-Pro & Bracket Format & Expert & 0.34/0.3336 \\
            & EM/F1 & Gemini-Pro & Linearized w/ Row Sign & Expert & 0.26/0.2686 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.21/0.05478 \\
            & EM/F1 & LLAMA-2-13B & Column Centric Json & Basic & 0.26/0.05106 \\
            & EM/F1 & LLAMA-2-13B & Row Centric Json & Basic & 0.24/0.05564 \\
            & EM/F1 & LLAMA-2-13B & Bracket Format & Basic & 0.21/0.04859 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/ Row Sign & Basic & 0.21/0.05244 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.21/0.04157 \\
            & EM/F1 & LLAMA-2-13B & Column Centric Json & CoT & 0.26/0.04127 \\
            & EM/F1 & LLAMA-2-13B & Row Centric Json & CoT & 0.24/0.0399 \\
            & EM/F1 & LLAMA-2-13B & Bracket Format & CoT & 0.23/0.03835 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/ Row Sign & CoT & 0.2/0.03636 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.26/0.04378 \\
            & EM/F1 & LLAMA-2-13B & Column Centric Json & Expert & 0.22/0.04644 \\
            & EM/F1 & LLAMA-2-13B & Row Centric Json & Expert & 0.3/0.04385 \\
            & EM/F1 & LLAMA-2-13B & Bracket Format & Expert & 0.29/0.04205 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.26/0.06868 \\
            & EM/F1 & LLAMA-2-70B & Column Centric Json & Basic & 0.29/0.09385 \\
            & EM/F1 & LLAMA-2-70B & Row Centric Json & Basic & 0.33/0.08039 \\
            & EM/F1 & LLAMA-2-70B & Bracket Format & Basic & 0.3/0.0734 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/ Row Sign & Basic & 0.29/0.09953 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.32/0.05196 \\
            & EM/F1 & LLAMA-2-70B & Column Centric Json & CoT & 0.33/0.05429 \\
            & EM/F1 & LLAMA-2-70B & Row Centric Json & CoT & 0.29/0.05785 \\
            & EM/F1 & LLAMA-2-70B & Bracket Format & CoT & 0.35/0.05678 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/ Row Sign & CoT & 0.3/0.06876 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.25/0.06812 \\
            & EM/F1 & LLAMA-2-70B & Column Centric Json & Expert & 0.25/0.07749 \\
            & EM/F1 & LLAMA-2-70B & Row Centric Json & Expert & 0.31/0.07292 \\
            & EM/F1 & LLAMA-2-70B & Bracket Format & Expert & 0.32/0.07476 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.21/0.04857 \\
            & EM/F1 & LLAMA-2-7B & Column Centric Json & Basic & 0.26/0.04963 \\
            & EM/F1 & LLAMA-2-7B & Row Centric Json & Basic & 0.26/0.05222 \\
            & EM/F1 & LLAMA-2-7B & Bracket Format & Basic & 0.22/0.05016 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/ Row Sign & Basic & 0.3/0.04725 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.24/0.03271 \\
            & EM/F1 & LLAMA-2-7B & Column Centric Json & CoT & 0.26/0.03668 \\
            & EM/F1 & LLAMA-2-7B & Row Centric Json & CoT & 0.24/0.03508 \\
            & EM/F1 & LLAMA-2-7B & Bracket Format & CoT & 0.26/0.04421 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/ Row Sign & CoT & 0.21/0.0333 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.22/0.04863 \\
            & EM/F1 & LLAMA-2-7B & Column Centric Json & Expert & 0.24/0.04803 \\
            & EM/F1 & LLAMA-2-7B & Row Centric Json & Expert & 0.29/0.04167 \\
            & EM/F1 & LLAMA-2-7B & Bracket Format & Expert & 0.23/0.04469 \\
            \midrule
\multirow{87}*{Totto} 
& bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.0846/0.4322/1.233/0.433 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Column Centric Json & Basic & 0.09453/0.4412/1.36/0.4546 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Row Centric Json & Basic & 0.08377/0.4311/1.272/0.4312 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Bracket Format & Basic & 0.08776/0.43/1.274/0.4418 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.0874/0.4156/1.228/0.4225 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.07918/0.4287/1.224/0.4269 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Column Centric Json & CoT & 0.09404/0.44/1.34/0.4391 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Row Centric Json & CoT & 0.07666/0.4222/1.212/0.4229 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Bracket Format & CoT & 0.08574/0.4301/1.249/0.4388 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.08354/0.4166/1.21/0.4205 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.07948/0.4442/1.194/0.4136 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Column Centric Json & Expert & 0.08118/0.4333/1.2/0.4109 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Row Centric Json & Expert & 0.07972/0.4359/1.159/0.4077 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Bracket Format & Expert & 0.07766/0.4366/1.182/0.4167 \\
            & bleu/meteor/nist/rougeL & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.07769/0.4307/1.142/0.401 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/o Row Sign & Basic & 0.08135/0.4634/1.314/0.4389 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Column Centric Json & Basic & 0.08882/0.478/1.363/0.4552 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Row Centric Json & Basic & 0.08798/0.4757/1.354/0.451 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Bracket Format & Basic & 0.08019/0.4722/1.375/0.4493 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/ Row Sign & Basic & 0.08869/0.4695/1.353/0.4459 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/o Row Sign & CoT & 0.08677/0.4685/1.325/0.4354 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Column Centric Json & CoT & 0.08683/0.4679/1.341/0.4424 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Row Centric Json & CoT & 0.08914/0.4782/1.368/0.4519 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Bracket Format & CoT & 0.08501/0.4661/1.323/0.455 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/ Row Sign & CoT & 0.08396/0.474/1.332/0.437 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/o Row Sign & Expert & 0.07765/0.4638/1.265/0.4276 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Column Centric Json & Expert & 0.08481/0.4663/1.29/0.431 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Row Centric Json & Expert & 0.08224/0.4706/1.266/0.4309 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Bracket Format & Expert & 0.07968/0.4467/1.239/0.4302 \\
            & bleu/meteor/nist/rougeL & GPT-4 & Linearized w/ Row Sign & Expert & 0.07287/0.4597/1.255/0.4272 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.08324/0.4201/1.297/0.4237 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Column Centric Json & Basic & 0.09645/0.441/1.397/0.4452 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Row Centric Json & Basic & 0.08672/0.431/1.317/0.4373 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Bracket Format & Basic & 0.1139/0.4535/1.379/0.448 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/ Row Sign & Basic & 0.08902/0.4427/1.346/0.4321 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.1106/0.4583/1.388/0.4447 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Column Centric Json & CoT & 0.1013/0.4529/1.352/0.4512 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Row Centric Json & CoT & 0.09812/0.4662/1.415/0.4506 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Bracket Format & CoT & 0.1038/0.4379/1.344/0.4392 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/ Row Sign & CoT & 0.09271/0.4561/1.382/0.4418 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.09485/0.4422/1.345/0.4237 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Column Centric Json & Expert & 0.1011/0.4563/1.38/0.4479 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Row Centric Json & Expert & 0.09874/0.4473/1.331/0.4341 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Bracket Format & Expert & 0.1011/0.447/1.37/0.4408 \\
            & bleu/meteor/nist/rougeL & Gemini-Pro & Linearized w/ Row Sign & Expert & 0.09521/0.4366/1.332/0.4251 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.02757/0.3413/0.6257/0.2292 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Column Centric Json & Basic & 0.02372/0.3295/0.5761/0.2274 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Row Centric Json & Basic & 0.01684/0.3046/0.5389/0.2192 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Bracket Format & Basic & 0.03253/0.3396/0.6142/0.248 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/ Row Sign & Basic & 0.03185/0.3192/0.5715/0.222 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.02931/0.3454/0.5844/0.2277 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Column Centric Json & CoT & 0.02401/0.328/0.5512/0.2149 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Row Centric Json & CoT & 0.02926/0.3337/0.5605/0.2253 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Bracket Format & CoT & 0.03133/0.3457/0.6101/0.2402 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/ Row Sign & CoT & 0.02648/0.3286/0.5649/0.2228 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.02484/0.3348/0.5733/0.2223 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Column Centric Json & Expert & 0.02434/0.3188/0.542/0.2078 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Row Centric Json & Expert & 0.02537/0.3178/0.5517/0.2145 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-13B & Bracket Format & Expert & 0.02572/0.344/0.5911/0.2308 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.04527/0.3517/0.7493/0.2718 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Column Centric Json & Basic & 0.0571/0.361/0.8273/0.3009 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Row Centric Json & Basic & 0.04871/0.3743/0.8237/0.2938 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Bracket Format & Basic & 0.04812/0.3736/0.7955/0.2886 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/ Row Sign & Basic & 0.04617/0.3611/0.757/0.283 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.04505/0.3623/0.7269/0.2744 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Column Centric Json & CoT & 0.04302/0.3648/0.7817/0.2879 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Row Centric Json & CoT & 0.04414/0.3546/0.7106/0.2686 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Bracket Format & CoT & 0.05112/0.3884/0.8134/0.2957 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/ Row Sign & CoT & 0.03486/0.3573/0.7112/0.2798 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.04/0.3568/0.6759/0.2625 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Column Centric Json & Expert & 0.01182/0.1303/0.2751/0.1032 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Row Centric Json & Expert & 0.04235/0.3514/0.6984/0.2703 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-70B & Bracket Format & Expert & 0.0463/0.3913/0.7676/0.2911 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.02824/0.3065/0.5672/0.2163 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Column Centric Json & Basic & 0.03684/0.3277/0.5724/0.2207 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Row Centric Json & Basic & 0.02523/0.3119/0.5458/0.2216 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Bracket Format & Basic & 0.03017/0.3396/0.5943/0.2357 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/ Row Sign & Basic & 0.02467/0.2914/0.4691/0.1906 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.02309/0.3071/0.4932/0.1984 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Column Centric Json & CoT & 0.02882/0.3205/0.5879/0.2207 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Row Centric Json & CoT & 0.02772/0.3231/0.5714/0.2283 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Bracket Format & CoT & 0.03136/0.3305/0.5877/0.2326 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/ Row Sign & CoT & 0.02197/0.2962/0.4737/0.1914 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.02851/0.301/0.5154/0.2067 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Column Centric Json & Expert & 0.02497/0.3126/0.4921/0.1986 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Row Centric Json & Expert & 0.02627/0.3108/0.5344/0.214 \\
            & bleu/meteor/nist/rougeL & LLAMA-2-7B & Bracket Format & Expert & 0.02536/0.333/0.5595/0.2229 \\
            \midrule
\multirow{87}*{WikiTableQuestions} 
& EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & Basic & 0.63/0.1296 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & Basic & 0.6/0.1121 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & Basic & 0.58/0.1314 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & Basic & 0.65/0.136 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & Basic & 0.58/0.1214 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & CoT & 0.68/0.07945 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & CoT & 0.72/0.03868 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & CoT & 0.72/0.0683 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & CoT & 0.67/0.04985 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & CoT & 0.68/0.06259 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/o Row Sign & Expert & 0.62/0.1182 \\
            & EM/F1 & GPT-3.5-Turbo & Column Centric Json & Expert & 0.62/0.08776 \\
            & EM/F1 & GPT-3.5-Turbo & Row Centric Json & Expert & 0.63/0.1179 \\
            & EM/F1 & GPT-3.5-Turbo & Bracket Format & Expert & 0.6/0.1104 \\
            & EM/F1 & GPT-3.5-Turbo & Linearized w/ Row Sign & Expert & 0.63/0.1105 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & Basic & 0.71/0.1671 \\
            & EM/F1 & GPT-4 & Column Centric Json & Basic & 0.75/0.1778 \\
            & EM/F1 & GPT-4 & Row Centric Json & Basic & 0.76/0.1851 \\
            & EM/F1 & GPT-4 & Bracket Format & Basic & 0.71/0.1766 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & Basic & 0.71/0.1736 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & CoT & 0.76/0.1679 \\
            & EM/F1 & GPT-4 & Column Centric Json & CoT & 0.76/0.1508 \\
            & EM/F1 & GPT-4 & Row Centric Json & CoT & 0.73/0.1624 \\
            & EM/F1 & GPT-4 & Bracket Format & CoT & 0.75/0.1576 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & CoT & 0.77/0.1681 \\
            & EM/F1 & GPT-4 & Linearized w/o Row Sign & Expert & 0.74/0.1493 \\
            & EM/F1 & GPT-4 & Column Centric Json & Expert & 0.73/0.1467 \\
            & EM/F1 & GPT-4 & Row Centric Json & Expert & 0.73/0.1585 \\
            & EM/F1 & GPT-4 & Bracket Format & Expert & 0.66/0.1468 \\
            & EM/F1 & GPT-4 & Linearized w/ Row Sign & Expert & 0.73/0.1541 \\
            & EM/F1 & Gemini-Pro & Linearized w/o Row Sign & Basic & 0.46/0.3788 \\
            & EM/F1 & Gemini-Pro & Column Centric Json & Basic & 0.34/0.2736 \\
            & EM/F1 & Gemini-Pro & Row Centric Json & Basic & 0.52/0.4312 \\
            & EM/F1 & Gemini-Pro & Bracket Format & Basic & 0.48/0.4243 \\
            & EM/F1 & Gemini-Pro & Linearized w/ Row Sign & Basic & 0.42/0.3403 \\
            & EM/F1 & Gemini-Pro & Linearized w/o Row Sign & CoT & 0.65/0.03457 \\
            & EM/F1 & Gemini-Pro & Column Centric Json & CoT & 0.61/0.03335 \\
            & EM/F1 & Gemini-Pro & Row Centric Json & CoT & 0.71/0.03854 \\
            & EM/F1 & Gemini-Pro & Bracket Format & CoT & 0.69/0.03843 \\
            & EM/F1 & Gemini-Pro & Linearized w/ Row Sign & CoT & 0.68/0.03402 \\
            & EM/F1 & Gemini-Pro & Linearized w/o Row Sign & Expert & 0.33/0.1993 \\
            & EM/F1 & Gemini-Pro & Column Centric Json & Expert & 0.3/0.1952 \\
            & EM/F1 & Gemini-Pro & Row Centric Json & Expert & 0.44/0.3293 \\
            & EM/F1 & Gemini-Pro & Bracket Format & Expert & 0.39/0.3078 \\
            & EM/F1 & Gemini-Pro & Linearized w/ Row Sign & Expert & 0.33/0.2025 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/o Row Sign & Basic & 0.4/0.03877 \\
            & EM/F1 & LLAMA-2-13B & Column Centric Json & Basic & 0.26/0.0296 \\
            & EM/F1 & LLAMA-2-13B & Row Centric Json & Basic & 0.31/0.04425 \\
            & EM/F1 & LLAMA-2-13B & Bracket Format & Basic & 0.35/0.04073 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/ Row Sign & Basic & 0.48/0.04624 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/o Row Sign & CoT & 0.43/0.03448 \\
            & EM/F1 & LLAMA-2-13B & Column Centric Json & CoT & 0.33/0.02486 \\
            & EM/F1 & LLAMA-2-13B & Row Centric Json & CoT & 0.4/0.02868 \\
            & EM/F1 & LLAMA-2-13B & Bracket Format & CoT & 0.43/0.03389 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/ Row Sign & CoT & 0.41/0.02725 \\
            & EM/F1 & LLAMA-2-13B & Linearized w/o Row Sign & Expert & 0.31/0.02934 \\
            & EM/F1 & LLAMA-2-13B & Column Centric Json & Expert & 0.31/0.02984 \\
            & EM/F1 & LLAMA-2-13B & Row Centric Json & Expert & 0.4/0.04904 \\
            & EM/F1 & LLAMA-2-13B & Bracket Format & Expert & 0.4/0.04067 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/o Row Sign & Basic & 0.41/0.05935 \\
            & EM/F1 & LLAMA-2-70B & Column Centric Json & Basic & 0.42/0.05406 \\
            & EM/F1 & LLAMA-2-70B & Row Centric Json & Basic & 0.49/0.07907 \\
            & EM/F1 & LLAMA-2-70B & Bracket Format & Basic & 0.44/0.07028 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/ Row Sign & Basic & 0.43/0.0759 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/o Row Sign & CoT & 0.49/0.05157 \\
            & EM/F1 & LLAMA-2-70B & Column Centric Json & CoT & 0.39/0.03203 \\
            & EM/F1 & LLAMA-2-70B & Row Centric Json & CoT & 0.66/0.05846 \\
            & EM/F1 & LLAMA-2-70B & Bracket Format & CoT & 0.59/0.04201 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/ Row Sign & CoT & 0.53/0.05709 \\
            & EM/F1 & LLAMA-2-70B & Linearized w/o Row Sign & Expert & 0.49/0.06216 \\
            & EM/F1 & LLAMA-2-70B & Column Centric Json & Expert & 0.43/0.04568 \\
            & EM/F1 & LLAMA-2-70B & Row Centric Json & Expert & 0.53/0.07346 \\
            & EM/F1 & LLAMA-2-70B & Bracket Format & Expert & 0.49/0.05788 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/o Row Sign & Basic & 0.39/0.04537 \\
            & EM/F1 & LLAMA-2-7B & Column Centric Json & Basic & 0.33/0.03959 \\
            & EM/F1 & LLAMA-2-7B & Row Centric Json & Basic & 0.33/0.04039 \\
            & EM/F1 & LLAMA-2-7B & Bracket Format & Basic & 0.37/0.04906 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/ Row Sign & Basic & 0.43/0.04305 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/o Row Sign & CoT & 0.45/0.03611 \\
            & EM/F1 & LLAMA-2-7B & Column Centric Json & CoT & 0.27/0.02566 \\
            & EM/F1 & LLAMA-2-7B & Row Centric Json & CoT & 0.46/0.03943 \\
            & EM/F1 & LLAMA-2-7B & Bracket Format & CoT & 0.43/0.03357 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/ Row Sign & CoT & 0.41/0.03181 \\
            & EM/F1 & LLAMA-2-7B & Linearized w/o Row Sign & Expert & 0.4/0.04252 \\
            & EM/F1 & LLAMA-2-7B & Column Centric Json & Expert & 0.3/0.03501 \\
            & EM/F1 & LLAMA-2-7B & Row Centric Json & Expert & 0.33/0.03816 \\
            & EM/F1 & LLAMA-2-7B & Bracket Format & Expert & 0.4/0.04313 \\
            \midrule

			\bottomrule
		\end{tabular}
		\end{adjustbox}
	\caption{all results}
	\label{tab:multitask-results}
\end{table*}
